Cryptographically Enforced Control Flow Integrity

Recent Pwn2Own competitions have demonstrated the continued effectiveness of control hijacking attacks despite deployed countermeasures including stack canaries and ASLR. A powerful defense called Control flow Integrity (CFI) offers a principled approach to preventing such attacks. However, prior CFI implementations use static analysis and must limit protection to remain practical. These limitations have enabled attacks against all known CFI systems, as demonstrated in recent work. This paper presents a cryptographic approach to control flow integrity (CCFI) that is both fine-grain and practical: using message authentication codes (MAC) to protect control flow elements such as return addresses, function pointers, and vtable pointers. MACs on these elements prevent even powerful attackers with random read/write access to memory from tampering with program control flow. We implemented CCFI in Clang/LLVM, taking advantage of recently available cryptographic CPU instructions. We evaluate our system on several large software packages (including nginx, Apache and memcache) as well as all their dependencies. The cost of protection ranges from a 3-18% decrease in request rate.

==> attacks.tex <==
\section{Possible Attacks}
\label{sec:attacks}

Like all other CFI systems that we are aware of, both fine-grain and 
course-grain, we only protect edges of the call-graph with the extra 
requirement that pointers must reside on the same address for a replay attack 
to be possible.  The use of the address where a pointer is stored, is something 
only possible at runtime and thus no other CFI system can build this securely.  
In this Section we will discuss address aliasing issues and potential future 
work to mitigate this, extending protection beyond a single edge of the call 
graph, and two potential data attacks that can affect control flow integrity.

\subsection{Address Aliasing}

Our weakest design point is that two different pointers may be stored at the 
same address, and an attacker could swap those pointers if he happens to have 
observed both of them and their corresponding MACs.  The randomization of stack 
and heap layout helps to mitigate this by reducing the probability that 
pointers alias to the same address.  Also return addresses and function 
pointers use different MAC schemes making them fundamentally incompatible.

One way future work could strengthen this is to use a slab allocator to store 
objects of the same type in the same virtual address space without any possible 
overlap with other objects.  As pointed out in our ideal model this can over be 
difficult and some types hide the full type information to be able to implement 
this.  Randomization could be used for the types we cannot reason about.  
Lastly, types that do not contain sensitive pointers may be a shared heap.

Another avenue for improving the defense is to add a hash of the type signature 
of functions into macptr and checkptr.  This would prevent two pointers of 
different types from being swapped as the type signature hash would be 
statically defined in the code using and creating pointers.  This doesn't 
prevent pointers with the same type signature and very different meanings from 
being swapped.

\subsection{Return Stack Chaining}

The return stack is the most vulnerable to address aliasing and sophisticated 
stack smashing attacks involving modifying multiple frames.  Our current design 
like all other CFI systems protects individual edges of the call graph, and not 
the entire chain.  Thus attackers may find useful replay attacks of sensitive 
pointers.

One approach would be to store a few return addresses in registers.  When the 
registers reserved are all full we would batch MAC and store these values on 
the stack.  This optimization allows us to exploit parallelism available in the 
AES-NI implementation.  We could see as much as a four time reduction in stack 
protection costs.

Another way to defend the return stack is to use hardware performance counters 
to verify the integrity of the return stack.  This by itself has been done in 
previous work~\cite{bib:kbouncer} to have the operating system kernel check the 
last few stack frames.  The technique could be applied to user level, but at an 
increased cost to the function epilogue.

These techniques could help us defend against more sophisticated stack smashing 
attacks without the need for randomization.  Potentially by doing a more 
expensive MAC computation.  It may also be practical to verify integrity of the 
entire stack, rather than each frame at a time.  This would allow us to detect 
partial replacements of several stack frames by attackers.

\subsection{Oracle Functions}

Our implementation computes MACs inline, and we desire to have no function 
where controlling the arguments to that function could generate a valid MAC for 
a given pointer.  We call these functions oracle functions and care has to be 
taken to avoid them.  Programmers may create oracle functions inadvertently 
through casting.  Our static analyzer checks for casting of sensitive pointers, 
which may also lead to MAC failures if copied around.

\subsection{Pointer Table Indices}

Our last avenue for attack is program data that can modify control flow.  We do 
not defend against this in any way.  Developers should use our macptr and 
checkptr primitives to protect indices into function tables, state machine 
variables, and critical conditional values (i.e.,\ whether a connection is 
authenticated or not).  A nice property that will aid the developer is that if 
a MAC is never witnessed by an attacker then a replay attack is not possible.  
This implies that if a variable is set to unauthenticated, the attacker cannot 
create a MAC for the authenticated variable without executing through the code 
that generates it.



==> hard.tex <==
%\subsection{Ideal Design}
\label{sec:hard}

Our current MAC design enforces control flow by protecting individual nodes in the
call graph and preventing replay attacks such that two nodes can never be
swapped.  An alternative design is to protect all edges of the control graph
without being concerned about replay (and swapping) of individual nodes.  This
more idealistic model for providing control flow integrity would depend on using
a MAC to protect the stack.  The key and a root key both must be kept secret in
registers.  On every function entry we would MAC the return pointer, frame
pointer, and the previous MAC.  Including the previous MAC allows the return
stack to form a Merkle tree of hashes.  The root of that tree is the root key.
Function epilogues would have to verify the entire call chain.  The Merkle tree
in combination with a root value stored safely in a register prevents any return
address from being replaced by a previously seen address stored at the same
location.  The requirement to verify the Merkle tree prevents attackers changing
a return value and MAC in the hierarchy to execute a function pointer previously
stored on the stack by a different function.

Function pointers on the stack as locals would have to be protected by a MAC
and also part of the same Merkle tree as the stack.  Applications often pass
locals on the stack including objects containing function pointers as
arguments.  The verification of a function pointer stored on the stack would
require walking the stack to verify the Merkle tree.  The pointers would be
unique not just to where they are stored but also the call chain that
constructed them.

Furthermore heap pointers, including vtables and other sensitive pointers, must
depend on a MAC that includes the address they are stored at so they cannot be
moved around.  An allocator similar to slab allocator~\cite{bib:slaballoc}
would guarantee that function pointers of different types never overlap.  For
example if we have two structures {\tt struct HTTPPlugin} and {\tt struct
ThreadPlugin} both containing function pointers we must guarantee that the heap
always keep the two types in separate memory pools.  Within each pool the
alignment of structures must be constant as it is dangerous if two different
method pointers align.  This is different from relying on randomness, as per our
current design.

This model protects control flow integrity, but is not practical.  Verifying
the entire call stack for every function prologue is too costly.  Similarly,
for function pointers stored as locals they will also be too expensive.  A slab
allocator-like heap is possible to build but in practice C program's cannot
statically determine types at compile time to build these slabs.  Tasks such as
casting objects to void pointers and memcpy'ing objects into buffers contained
in other objects (thus hiding the type information) are examples of why this is
tricky if not impossible to do at compile time.

Our design attempts to achieve practical trade-offs using a mixture of
randomization and cryptography to make attacks impractical.


